Experimental Demonstration of Over the Air Federated Learning for Cellular Networks

Over-the-air federated learning (OTA-FL) offers an exciting new direction over classical FL by averaging model weights using the physics of analog signal propagation. Since each participant broadcasts its model weights concurrently in time and frequency, this paradigm conserves communication bandwidth and model upload latency. Despite its potential, there is no prior large-scale demonstration on a real-world experimental platform. This paper proves for the first time that OTA-FL can be deployed in a cellular network setting within the constraints of a 5G compliant waveform. To achieve this, we identify challenges caused by multi-path fading effects, thermal noise at the radio devices, and maintaining highly precise synchronization across multiple clients to perform coherent OTA combining. To address these challenges, we propose a unified framework for real-time channel estimation, model weight to OFDM symbol mapping and dual-layer synchronization interface to perform OTA model training. We experimentally validate OTA-FL using two relevant applications - Channel Estimation and Object Classification, at a large-scale on ORBIT Testbed and a portable setup respectively, along with analyzing the benefits from the perspective of a telecom operator. Under specific experimental conditions, OTA-FL achieves equivalent model performance, supplemented with 43 times improvement in spectrum utilization and 7 times improvement in energy efficiency over classical FL when considering 5 nodes.

==> sections/unused.tex <==
\section{$\name$ Framework}
\label{sec:framework}
\add{Suyash, Debashri}

\subsection{Data Acquisition}
\label{subsec:data_acqu_and_preprocessings}
The position and 3-D map of the surroundings is collected by the co-operative vehicles using the GPS and LiDAR sensory unit and passed through the following preprocessing steps

\subsubsection{Structuring and Quantizing LiDAR data}
\label{sec:preprocessing_lidar}
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Lidar_coordination.png}
    \caption{The proposed Lidar point cloud acquisition and preprocessing method in $\name$. We only show the quantization involving 2 RSUs for simplicity.}
    % (-1,-2,-3) for each transmitter and -4 for the ego car to identify it has the receiver, obstacles as 1
    \label{fig:LIDAR_feature_ext}
    \vspace*{-10pt}
\end{figure} 

The LiDAR point clouds are an unordered set of points in a three-dimensional space. The characteristic that prohibits us from leveraging popular Convolutional Neural Networks (CNN) architectures to LiDAR point clouds is their permutation invariance, implying that varying the order of point clouds will still represent the same scene. On the contrary, CNNs have been designed to process ordered grid structures like image pixels, where changing the order of pixels will modify the scene being represented. Hence, we need to convert our LiDAR point clouds into a similar ordered grid structure to represent the 3-D space. We build a 3-D quantized cuboid structure to represent the spatial extent of the effective LiDAR range, with each individual unit called as voxel (3-D equivalent of pixel) to store the point cloud occupancy in that region. The voxels containing at least one point cloud are marked as 1 to signify the presence of obstacles in that region whereas unoccupied voxels are stored with 0. We derive the position of the ego car from the GPS co-ordinates and label the corresponding voxel as -4 to signify the receiver location. Similarly, we label the voxels containing the RSUs as -1, -2 and -3 to allow the model identify the 3 candidate transmitters available in that region. 

% Copied from the TVT paper, please update
% \fix{Suyash} {\color{red} Suyash, please write this part following the gray texts, and tune as per settings of this paper.} {\color{gray}To process the LiDAR data, we first construct a quantized view of the spatial extent of the surroundings. This data structure resembles a stack of cuboid regions placed adjacent to each other.The LiDAR point clouds reside in the cuboid regions according to their relative  distances as measured from a shared origin as in~\cite{dias2019position}. We mark the cuboids that contain blocking obstacles using label 1. Since we know the coordinates of the Tx and Rx, we label the cuboids containing them as -1 and -2, respectively. The LiDAR preprocessing happens at the vehicle. Thus, the RSUs must share its location in downlink with the vehicles. This can be done when the vehicles check in with the RSUs. The raw LiDAR point cloud is a collection of $(x,y,z)$ points that correspond to the location of detected objects in the environment. Directly exploiting the raw point cloud (with varying number of points depending on traffic density) not only comes with huge computational cost but also raises ML architecture design challenges as the input to a neural network must be preferably fixed in size. Hence, we use a preprocessing step as shown in Fig. \ref{fig:LIDAR_feature_ext} first proposed in~\cite{klautau2019} that considers a limited spatial zone for each axis. This space corresponds to coverage range of BS and is  denoted as $(X_{\min},X_{\max})$, $(Y_{\min},Y_{\max})$, and $(Z_{\min},Z_{\max})$. Then, we construct a 3-D histogram that corresponds to a quantized 3-D representation of the space. The histogram bin size along the three spatial dimensions $(b_x,b_y,b_z)$ can be set based on desired resolution. The LiDAR point clouds lie in the corresponding bins of the histogram based on their location. Since the BS is fixed in our setting, it always occupies the same cell of the histogram with indicator ($-2$). The corresponding cell of the target receiver is also acquired with GPS data and indicated with ($-1$). The remaining elements are mapped to the corresponding histogram elements with ($1$), which implies the presence of obstacles. This leads to a compact 3-D representation of the environment that we use as input for our pipeline. } %

\subsubsection{Co-ordinate System}
We follow a pre-defined global co-ordinate system where all connected and autonomous vehicles (CAVs) will project their LiDAR point clouds, to avoid complicated co-ordinate transformations during the fusion process. The GPS data contains the latitude and longitude co-ordinates in degrees, whereas the LiDAR data and further distance based processing will be efficient if we have the locations transformed to a Cartesian co-ordinate system. Thus, we define a fixed origin for the entire space to ensure a unified co-ordinate system for all the co-operative cars. Regarding the LiDAR point clouds, each car records the data considering the LiDAR sensor location as the local origin point and projects it to the global co-ordinate system, followed by the quantization process mentioned in the previous section.

% We need this section.. 
\noindent {\bf Notations of the Data Matrices: }As mentioned in Sec.~\ref{subsec:problem_formualtion}, we consider $\{\vcl\}_{i=1}^{\numvcl}$ vehicles and $\{\rsu\}_{j=1}^{\numrsus}$ RSUs in the environment. In $\name$, the vehicles are considered either by: (a) {\em Ego} vehicle which is our vehicle of interest, (b) the vehicles which are front of the Ego vehicle, named as {\em front} CAV, and (c) the ones which are back of the Ego vehicle, named as {\em back} CAV. the vehicles in consider the Ego vehicle $\vcl_{e}$ and a number of CAVs \{${\vcl_1}, {\vcl_2} \cdots {\vcl_{\numvcl}}\}$ in a particular region. To the Ego vehicle $\vcl_{e}$, all the \{${\vcl_1}, {\vcl_2} \cdots {\vcl_{\numvcl}}\}$ CAVs are seen as either front CAVs or back CAVs. We denote the two sets as \{${\vcl^f_1}, {\vcl^f_2} \cdots {\vcl^f_{\numvcl_f}}\}$ and \{${\vcl^b_1}, {\vcl^b_2} \cdots {\vcl^b_{\numvcl_b}}\}$, where $\numvcl_f + \numvcl_b + 1 = \numvcl$, and $\{\vcl^f\}_{i=1}^{\numvcl_f}+ \{\vcl^b\}_{i=1}^{\numvcl_b} = \{\vcl\}_{i=1}^{\numvcl}$. The Ego vehicle $\vcl_{e}$ wants to establish a link with an optimal RSU.

We denote the Ego and $ith$ front and back vehicles as $\vcl_e$, $\vcl^f_i$, and $\vcl^b_i$, respectively. We also denote and $jth$ RSU as $\rsu_j$. We define the data matrices for the quantized Lidar data at $\vcl_e$, $\vcl^f_i$, and $\vcl^b_i$ vehicles as: $X^{\vcl_e}_{\ldr}\in \mathbb{R}^{d_0^{\vcl_e} \times d_1^{\vcl_e} \times d_2^{\vcl_e}}$, $X^{\vcl^f_i}_{\ldr}\in \mathbb{R}^{d_0^{\vcl^f_i} \times d_1^{\vcl^f_i} \times d_2^{\vcl_e}}$, and $X^{\vcl^b_i}_{\ldr}\in \mathbb{R}^{d_0^{\vcl^b_i} \times d_1^{\vcl^b_i} \times d_2^{\vcl^b_i}}$ where $(d_0^{\vcl_e} \times d_1^{\vcl_e} \times d_2^{\vcl_e})$, $(d_0^{\vcl^f_i} \times d_1^{\vcl^f_i} \times d_2^{\vcl^f_i})$ , and $(d_0^{\vcl^b_i} \times d_1^{\vcl^b_i} \times d_2^{\vcl^b_i})$  are the dimensionalities of preprocessed Lidar data at the Ego, front, back vehicles, respectively. 


% We denote the $ith$ vehicle as $\vcl_i$, and $jth$ RSU as $\rsu_j$. We define the data matrices for the quantized Lidar data at $\vcl_i$ as: $X^{\vcl_i}_{\ldr}\in \mathbb{R}^{N^{\vcl_i}_t\times d_0^{\vcl_i} \times d_1^{\vcl_i} \times d_2^{\vcl_i}}$, where $N^{\vcl_i}_t$ is the number of training samples and $(d_0^{\vcl_i} \times d_1^{\vcl_i} \times d_2^{\vcl_i})$ is the dimensionality of preprocessed LiDAR data at the Ego vehicle $\vcl_i$. 



%\noindent {\bf Motivation for co-operative perception:} Talk about why cooperative perception is better and refer to Fig.~\ref{fig:cooperative_perception_motivation}.
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Harbor_figure_2.png}
    \caption{A LiDAR point cloud example showing the benefits
of collaborative sensing by merging a nearby vehicle’s data
(green) to a single vehicle (blue)..{\color{red}we need similar figure}}
    \label{fig:cooperative_perception_motivation}
    \vspace*{-10pt}
\end{figure}

% This is a basic formulation, we give details later.. 
\subsection{Local Feature Extraction at Each Vehicle}
\label{subsec:feature_extraction} 

In this case, the other vehicles in the region will be eligible to serve as co-operating vehicles. Each vehicle will have a trained the same encoder network represented by $f_{\theta^{\vcl_i}_f}^\ldr$ and parameterized by weight vectors $\theta^{\vcl_i}_f$. %The structure of the encoder network is described in Fig.~\ref{fig:model_architectures}, comprising of Convolution operations to extract the local features and Max Pooling to down-sample and retain the most prominent values in the feature map. We include 3 residual blocks to include information learnt at prior layers to effectively flow through the network. 
The LiDAR quantization process will involve all the CAVs projecting their data to a common co-ordinate system, considered by ego vehicle ${\vcl_i}$. We perform the quantization process as described in the previous section. The only difference in the quantization of ego vehicle will be the position encoding of -4 to identify the location of the Receiver with respect to the surrounding RSUs. 
Once, we have the quantized LiDAR data, we perform feature extraction at each vehicle. {\color{blue} put it in the implementation details subsection.}

We denote the dimension of the extracted feature as $d^{\vcl_e}$, $d^{\vcl^f_i}$, and $d^{\vcl^b_i}$ for vehicle Ego vehicle ${\vcl_e}$, $ith$ front vehicle ${\vcl^f_i}$, and $ith$ back vehicle ${\vcl^b_i}$, respectively. The  feature extractors $f_{\theta^{\vcl_e}}^\ldr$, $f_{\theta^{\vcl^f_i}}^\ldr$, and $f_{\theta^{\vcl^b_i}}^\ldr$  map each sample input to dimension $d^{\vcl_e}$, $d^{\vcl^f_i}$, and $d^{\vcl^b_i}$, for Ego, front and back vehicles, respectively. We refer to the output of these feature extractors as the latent embedding of the LiDAR data at Ego, front and back vehicles. Formally,%
\begin{subequations}
    \begin{align}
      \mathbf{z}^{\vcl_e}_{\ldr} & = f_{\theta^{\vcl_e}}^\ldr(X^{\vcl_e}_{\ldr}),~f_{\theta^{\vcl_e}}^\ldr:\mathbb{R}^{N^{\vcl_e}_t\times d_0^{\vcl_e} \times d_1^{\vcl_e} \times d_2^{\vcl_e}} \mapsto \mathbb{R}^{d^{\vcl_e}}\\
      \mathbf{z}^{\vcl^f_i}_{\ldr}  &  = f_{\theta^{\vcl^f_i}}^\ldr(X^{\vcl^f_i}_{\ldr}),~f_{\theta^{\vcl^f_i}}^\ldr:\mathbb{R}^{N^{\vcl^f_i}_t\times d_0^{\vcl^f_i} \times d_1^{\vcl^f_i} \times d_2^{\vcl^f_i}} \mapsto \mathbb{R}^{d^{\vcl^f_i}}\\
      \mathbf{z}^{\vcl^b_i}_{\ldr} &  = f_{\theta^{\vcl^b_i}}^\ldr(X^{\vcl^b_i}_{\ldr}),~f_{\theta^{\vcl^b_i}}^\ldr:\mathbb{R}^{N^{\vcl^b_i}_t\times d_0^{\vcl^b_i} \times d_1^{\vcl^b_i} \times d_2^{\vcl^b_i}} \mapsto \mathbb{R}^{d^{\vcl^b_i}}   
    \end{align}
\label{eq:feature_extrs}%
\end{subequations}
where  $\mathbf{z}^{\vcl_e}_{\ldr}$, $\mathbf{z}^{\vcl^f_i}_{\ldr}$, and $\mathbf{z}^{\vcl^b_i}_{\ldr}$ show the extracted latent embeddings for the quantized Lidar data $X^{\vcl_e}_{\ldr}$, $X^{\vcl^f_i}_{\ldr}$, and $X^{\vcl^b_i}_{\ldr}$ for  Ego ${\vcl_e}$, front ${\vcl^f_i}$ and back ${\vcl^b_i}$ vehicles, respectively.

{\color{red} We can add the Bandwidth Aware Adaptive Feature story here}

% DR: commented as not performing well
% At this stage, we perform fusion at the Ego vehicle to obtain a broader perception of the environment. In  $\name$, we propose two ways of doing so by either using the quantized Lidar data or by leveraged extracted latent embeddings. 


% \noindent {\bf Na\"ive Fusion for Co-operative Perception: } In this method, $\name$ at the Ego vehicle collects all the quantized Lidar data from the neighboring vehicles. We perform a fusion of those quantized data at the Ego vehicle and generate a broader quantized perception of the environment $X_{\ldr}^{Q}$, represented by:
% \begin{align*}
%     X_{\ldr}^{Q} = \mathcal{F}(X^{\vcl_1}_{\ldr},\cdots,X^{\vcl_{\numvcl}}_{\ldr})\in \mathbb{R}^{d^{\vcl_1}+\cdots+d^{\vcl_{\numvcl}}}.
% \end{align*}
% where, $\numvcl$ is the total number of vehicle and $\mathcal{F}(.)$ is considered fusion strategy. The $\mathcal{F}(.)$ is concatenation of the inputs, represented by: $\mathcal{F}(X^{\vcl_1}_{\ldr},\cdots,X^{\vcl_{\numvcl}}_{\ldr}) = [X^{\vcl_1}_{\ldr};\cdots;X^{\vcl_{\numvcl}}_{\ldr}]$. 

\subsection{Spatial fusion at the Ego vehicle for co-operative perception}
\label{subsec:spatial_fusion}

{\color{red} Suyash, input features: $ \{\mathbf{z}^{\vcl_i}_{\ldr}\}_{i=1}^{\numvcl-1}$ output would be a set of selected vehicles $\vcl_S = \{\vcl_i\}_{i=1}^{i=\eta}$ with $\eta$ selected vehicles. Please use different notations, other than using $f$.. use like $\eta$, $\zeta$ etc. Need to represent {\em torch.bmm} in math form.}

We perform fusion at the Ego vehicle with the features from front and back vehicles to obtain a broader perception of the environment. In  $\name$, we propose to perform the spatial fusion by leveraging the extracted latent embeddings. 

The spatial fusion of the features from the co-operative cars involves computing a matching score to identify appropriate candidates and concatenate these supporting feature maps according to their computed similarity. Broadcasting the features from all co-operative vehicles irrespective of the necessity will result in a massive overhead and saturate the bandwidth. Therefore, we opt for a handshaking mechanisms where the ego car requests surrounding neighbours for support before the LiDAR quantization process. Thereafter, all cars extract their feature maps locally in a distributed manner. The supporting cars utilize V2V existing communication links to send their feature maps to the ego car using C-V2X protocol. 

\noindent {\bf Selecting the neighbours: } Traditional approaches like nearest neighbours or distance based selection with the intent to obtain the widest perception involves fully connected graphs which are not efficient as the number of CAVs scale up in the region. Hence, we opt in for an attention mechanism to identify the neighbours. Firstly, we compute a similarity score between the feature map of the ego vehicle and each of the co-operative CAV -
\[\mu = f(\vcl_e,  \vcl_i)\]

where f is the similarity function between feature map of ego car and supporting car. We use dot-product based attention as the similarity function owing to the ease of computation and effectiveness. If this value is greater than a pre-defined threshold, we consider this as a suitable neighbor for fusion.

\noindent {\bf Fusing the selected Feature Maps: } 
In $\name$, the fused feature vector consists of two components - one is the ego feature map and second is a weighted summation of the supporting feature maps, which are collectively concatenated with the ego feature map. We perform a softmax operation, denoted by $\sigma$, over all the similarity scores $\mu$ of the connecting agents to scale them between 0 to 1, followed by summing them as a weighted average.

\[w_i = \sigma(\mu)\]

\[f_i = \sum w_i * v_i\]

The intuition behind this is to keep the ego features intact by not modifying it as a part of the weighted average with other supporting cars. On the other hand, we do not perform a naive concatenation as we do not want to assign equal weight-age to the supporting cars and increase the complexity of the further layers of the Neural Network.

% \noindent {\bf Feature fusion for co-operative perception: }
% In this stage  $\mathbf{z}_{\vcl_i} \in\mathbb{R}^{d^{\vcl_i}}$ we fuse them in aggregated manner and generate the combined latent feature matrix $\mathbf{z}_{\ldr}$ as: 
% \begin{align*}
%     \mathbf{z}_{\ldr}^{F} = \mathcal{F}(\mathbf{z}_{\vcl_1};\cdots;\mathbf{z}_{\vcl_{\numvcl}})\in \mathbb{R}^{d^{\vcl_1}+\cdots+d^{\vcl_{\numvcl}}}.
% \end{align*}
% Similarly, the fusion strategy $\mathcal{F}(.)$ is represented as: $\mathcal{F}(\mathbf{z}_{\vcl_1},\cdots,\mathbf{z}_{\vcl_{\numvcl}}) = [\mathbf{z}_{\vcl_1};\cdots;\mathbf{z}_{\vcl_{\numvcl}}]$. 



\noindent {\bf Feature-based co-operative perception: }
In this stage, we have the latent embeddings $\mathbf{z}^{\vcl_e}_{\ldr}$, $\mathbf{z}^{\vcl^f_s}_{\ldr}$, and $\mathbf{z}^{\vcl^b_s}_{\ldr}$ from the  Ego ${\vcl_e}$, and selected front ${\vcl^f_s}$ and back ${\vcl^b_s}$ vehicles, respectively. The $\mathbf{z}^{\vcl_e}_{\ldr} \in\mathbb{R}^{d^{\vcl_e}}$, $\mathbf{z}^{\vcl^f_s}_{\ldr} \in\mathbb{R}^{d^{\vcl^f_s}}$, and $\mathbf{z}^{\vcl^b_s}_{\ldr} \in\mathbb{R}^{d^{\vcl^b_s}}$ . In $\name$, we fuse these latent embeddings in aggregated manner and generate the combined latent feature matrix $\mathbf{z}_{\ldr}$ as: 

\begin{equation}
% \begin{align}
    \mathbf{z}_{\ldr} = \mathcal{C}(\mathbf{z}^{\vcl_e}_{\ldr},\mathbf{z}^{\vcl^f_s}_{\ldr}, \mathbf{z}^{\vcl^b_s}_{\ldr})\in \mathbb{R}^{d^{\vcl_e}+d^{\vcl^f_s}+d^{\vcl^b_s}}.
% \end{align}
\end{equation}

The fusion strategy $\mathcal{C}(.)$ is represented as: $\mathcal{C}(\mathbf{z}^{\vcl_e}_{\ldr},\mathbf{z}^{\vcl^f_s}_{\ldr}, \mathbf{z}^{\vcl^b_s}_{\ldr}) = [\mathbf{z}^{\vcl_e}_{\ldr};\mathbf{z}^{\vcl^f_s}_{\ldr}; \mathbf{z}^{\vcl^b_s}_{\ldr}]$. 



% {\color{red}Suyash, please expand more, talk about what specific spatial fusion you are using, may be different representation of $\mathcal{C}(.)$. }

% We denote the aggregated fusion network as $f_{\theta^\AGF}^\AGF(\cdot)$:
% \begin{align*}
%  \scores_{\AGF} = \sigma (f_{\theta^\AGF}^\AGF(\mathbf{z})),~~~~~f_{\theta^\AGF}^\AGF:\mathbb{R}^{d^{\rad}+d^{\aco}+d^{\sei}} \mapsto \mathbb{R}^{|\mathcal{V}|} \end{align*}
%  where $\sigma$ is the sigmoid.

\subsection{RSU Prediction at the Ego Vehicle}
\label{subsec:rsu_prediction}
The last stage of the $\name$ framework is the real time prediction of the RSUs at each location for the Ego vehicle $\vcl_e$. The set of output labels are the RSUs within the environment: $\mathcal{L} = \{\rsu_1, \cdots , \rsu_{\numrsus}\}$, where $\numrsus$ is the total number of RSUs in the environment. The label matrix $Y_\rsu\in \{0,1\}^{\numrsus}$  represents the one-hot encoding of $\numrsus$ RSUs, where the optimum RSU for association is set to $1$, and rest are set to $0$ as per Eq.~\eqref{eq:best_rsu}. 

% DR: commented as not performing well
% The proposed NN-based classifier predicts the probability of each class using either the fused quantized data $X_{\ldr}^{Q}$, or fused features $\mathbf{z}_{\ldr}^{F}$. The neural network transformations for mapping such fused features to generate the label prediction is denoted as $q^{\ldr}_{\theta^{\vcl_i}_{q}}$ parameterized by $\theta^{\vcl_i}_{q}$ while using the fused quantized data and  $p^{\ldr}_{\theta^{\vcl_i}_{p}}$ parameterized by $\theta^{\vcl_i}_{p}$  while using the fused features.


% \noindent {\bf Neural network modeling leveraging na\"ive fusion: } The formal definition of the neural network which uses the fused quantized Lidar data, is presented as:
% \begin{equation} 
% \label{eq:classifier}
% \vspace*{-0.05in}
% \hat{Y}^{\rsu} =\sigma(q^{\ldr}_{\theta^{\vcl_i}_{q}}(X_{\ldr}^{Q})) ~~~~~~q^{\ldr}_{\theta^{\vcl_i}_{q}}:\mathbb{R}^{d^{\vcl_1}+\cdots+d^{\vcl_{\numvcl}}} \mapsto \mathbb{R}^{\numrsus}
% % \vspace*{-0.05in}
% \end{equation}
% where $\sigma$ is \emph{Softmax}.

The proposed NN-based classifier predicts the probability of each class using the fused features $\mathbf{z}_{\ldr}$. The neural network transformations for mapping such fused features to generate the label prediction at the Ego vehicle $\vcl_e$ is denoted as  $p^{\ldr}_{\theta^{\vcl_e}}$ parameterized by $\theta^{\vcl_e}$.


\noindent {\bf Neural network modeling leveraging feature fusion: } 
The formal definition of the neural network which uses the fused Lidar features with $\sigma$ as \emph{Softmax} activation, as:
\begin{equation} 
\label{eq:classifier}
\vspace*{-0.05in}
\hat{Y}^{\rsu} =\sigma(p^{\ldr}_{\theta^{\vcl_e}}(\mathbf{z}_{\ldr})) ~~~~p^{\ldr}_{\theta^{\vcl_e}}:\mathbb{R}^{d^{\vcl_e}+d^{\vcl^f_s}+d^{\vcl^b_s}} \mapsto \mathbb{R}^{\numrsus}
% \vspace*{-0.05in}
\end{equation}
% where $\sigma$ is \emph{Softmax}.


\noindent {\bf RSU prediction: } The predicted class index, $\hat{\rsu*}$, from the generated probability vector, $\hat{Y}^{\rsu}$, is defined as:
\begin{equation}
\label{eq:argmax}
% \vspace*{-0.05in}
    \hat{\rsu*} = \underset{0\leq \rsu \leq len(\mathbb{I})}{\arg\max}~(\hat{Y}^{\rsu})
    % \vspace*{-0.05in}
\end{equation}


